A Simple Global Neural Discourse Parser

Discourse parsing is largely dominated by greedy parsers with manually-designed features, while global parsing is rare due to its computational expense. In this paper, we propose a simple chart-based neural discourse parser that does not require any manually-crafted features and is based on learned span representations only. To overcome the computational challenge, we propose an independence assumption between the label assigned to a node in the tree and the splitting point that separates its children, which results in tractable decoding. We empirically demonstrate that our model achieves the best performance among global parsers, and comparable performance to state-of-art greedy parsers, using only learned span representations.

==> double.tex <==
\section{Double Training}\label{sec:double}

The core idea of this paper is to learn a shared
representation from different inference algorithms, \ie%
transition-based parsing and chart-based parsing.
The assumption behind this idea is that chart-based parsing and
transition-based parsing make different errors~\cite{mcdonald2007characterizing}.
% The learned shared representation can encode both information
% from chart parsing perspective and transition parsing
% perspective.

These two paring methods are completely different.
On one hand, transition parsing uses local training and greedy
inference but can utilize rich features of parsing
history.
On the other hand, chart parsing uses global training and
exact (or near exact) inference but can only utilize a
limited features of parsing history.
However, despite the difference, these two different kinds
of parsers can achieve similar performance but with different errors
(shown in \S\ref{sec:exp}).
This phenomenon suggests that these two parsers make
decisions based on different aspects of the trees.
An initutive idea is to combine them together to learn a
shared representations which can encode information from
both of these parsers.

This is different from multi-view
learning~\cite{wang2015deep,zhao2017multi} or
multi-task learning~\cite{ruder2017overview,LuongLSVK15}.
In multi-view learning, one data point is usually
represented by different sets of features and learn a joint
funtion to improve the generalization performance.
Here, we use the same feature representation but different inference
algorithms.
In multi-task learning, a common representation is shared by
the related but different tasks.
In this way, we expect the information comes from related
tasks can help the target task.
However, in this paper, the task is still the same, \ie%
parsing a document into a RST tree.
We learn a shared representation from differnt inference
algorithms.

\subsection{Combining Two Parsers}

In order to combien these two parsers, we need two
things:
\begin{itemize}
    \item A shared EDU representation.
    \item A joint loss function.
\end{itemize}
The shared EDU representation is described in
\S\ref{sec:rep}.
Here, we focus on the joint loss function.
We use $\ell_{chart}(T^{*})$ and $\ell_{sr}(T^{*})$ to
represent the loss of chart-based parser and
transition-based parser respectively.
A simple choice of joint loss function is to use weighted
sum of these two losses:
\begin{equation}
    \ell_{joint}(T^{*}) = \ell_{chart}(T^{*}) + \gamma\ell_{sr}(T^{*})
\end{equation}

where $\gamma$ is a hyper-parameter balancing the two
losses.
We can sum them up because two parsers use the same kind of loss
function (described in \S\ref{sec:chart} and
\S\ref{sec:transition}).



==> transition.tex <==
\section{Transition-based Parser}\label{sec:transition}
In this seciton, we will first describe the transition
system we used in this work.
Then, scoring function and loss functions are presented.

\subsection{Transition System}
Transition-based method aims at converting a tree into a
squence of actions, which makes the problem a
squence-to-squence problem~\cite{BahdanauCB14}.
It is conceptually simple and flexible in terms of
incorporating rich features, which is widely used by many
NLP
tasks~\cite{zhu2013fast,chen2014fast,dyer2015transition,zhang2016transition}.

We follow~\citet{ji2014representation} for our transition-based parser.
Our transition system consisits of two parts: states and
actions.
A state is used to store partial trees we have parsed and
an action is used to transform the state to next state.
One state consisits of a stack and a queue.
Initially, the stack is empty and the queue consisits of all the
EDUs of the input document.
There are two types of actions in this system:
\begin{itemize}
    \item SHIFT\@: Move the first EDU in the queue to the
        stack, forming a leaf node.
    \item REDUCE$(l,p)$: Merge the top two nodes of the
        stack and produce a new subtree whose children are
        these two nodes. $l$ is the relation label and
        $p\in\{NN,NS,SN\}$ indicates the nuclearity
        label (nuclear ($N$) or satellite ($S$)).
\end{itemize}

AT each step of parsing process, a classifier is used to
decide which action should be taken based on the current
state.

\subsection{Scoring and Loss Functions}

Suppose $\be_i$ represents the feature representations
(described in \S\ref{sec:rep}) of each
EDU $E_i$ in the document.
For $k^{th}$ subtree $sub_{k}$ in the stack, we concate the
representations of first and last EDUs that this subtree covers
as the representation of this subtree:
\begin{equation}
    \bh_{sub_k} = \be_i \oplus \be_j
\end{equation}
where $i$ and $j$ is the first and last indices of the EDU span
that this subtree convers.

Similarly, the representation of $k^{th}$ element $h_{q_k}$ in the queue is
simply the representation of EDU $\be_i$, where $i$ is the
EDU index in the document of this element.

We use the top $3$ elements of the stack and queue ($6$ in
total) as the representation of current state.
The final representation of a state $s$ is:
\begin{equation}
    \bh_s = \bh_{sub_0} \oplus \bh_{sub_1} \oplus \bh_{sub_2} \oplus
    \bh_{q_0} \oplus \bh_{q_1} \oplus \bh_{q_2}
\end{equation}

We use a feedforward classifier as the action predictor.
The input of this classifier is $\bh_s$ and output is the
scores of all possible actions.

Suppose $S(s,a)$ is the score of state and action pair $(s,a)$.
In order to be consistent with the loss funciton of chart
parsing (decsribed in \S\ref{sec:chart-loss}), we
use margin-based loss function for transition-based parsing.
We want the score of golden state-action pair $(s,a)$ is
higher than any other actions.
For each golden state-actin pair $(s,a^{*})$, the loss is defined as:
\begin{equation}
    \ell_{sr}(s,a^{*}) = \frac{1}{N}\sum\limits_{a\in\sA}^N
    \max\left(0, 1+ S(s,a) - S(s,a^{*})\right)
\end{equation}

where $\sA$ is the set of all possible actions and
$N$ is the size is $\sA$.

The overall loss for a golden tree $T^{*}$ is simply the sum
of the loss of all statet-action pairs in the tree $T^{*}$:
\begin{equation}
    \small
    \ell_{sr}(T^{*}) = \frac{1}{N}\sum\limits_{(s,a^{*})\in
    T^{*}}\sum\limits_{a\in\sA}^N
    \max\left(0, 1+ S(s,a) - S(s,a^{*})\right)
\end{equation}

